Consistent Multimodal Generation via A Unified GAN Framework

We investigate how to generate multimodal image outputs, such as RGB, depth, and surface normals, with a single generative model. The challenge is to produce outputs that are realistic, and also consistent with each other. Our solution builds on the StyleGAN3 architecture, with a shared backbone and modality-specific branches in the last layers of the synthesis network, and we propose per-modality fidelity discriminators and a cross-modality consistency discriminator. In experiments on the Stanford2D3D dataset, we demonstrate realistic and consistent generation of RGB, depth, and normal images. We also show a training recipe to easily extend our pretrained model on a new domain, even with a few pairwise data. We further evaluate the use of synthetically generated RGB and depth pairs for training or fine-tuning depth estimators. Code will be available at https://github.com/jessemelpolio/MultimodalGAN.

==> figure_latex/image_inversion.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/image_inversion1.pdf}
\end{center}
\vspace{-4mm}
\caption{Results of image inversion with our three-modality model. Inverting RGB only obtains its depth and normal for free.}
\label{fig:image_inversion}
\vspace{-6mm}
\end{figure}

==> figure_latex/main_diagram.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=1.02\linewidth]{figures/main_diagram.pdf}
\end{center}
\caption{Architecture of our generator (a) and discriminators (b).\soren{moving the 'a', 'b' labels under the image into the image would save space.}}
\label{fig:main_diagram}
\end{figure*}

==> figure_latex/teaser.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{figures/teaser_image.pdf}
\end{center}
\caption{Generated samples by our model. The first row is RGB images and the second and third rows represent the corresponding depth maps and surface normals. These samples covers diverse classes in Stanford2D3D dataset~\cite{armeni2017stanford2d3d}.}
\label{fig:teaser}
\end{figure*}

% The generator $G$ starts from a random vector $z$ sampled from normal distribution and generates multi-modality outputs, \ie, RGB (1st row), depth map (2nd row) and surface normal (3rd row) in this case.

==> tables/depth_estimation.tex <==
\begin{table}[t]
  \caption{Results of using our generator to augment data for depth estimation. Perc. real (\%) means percentage of real data used for training. Likewise, Perc. gen. is the percentage of generated data used. Percentage is calculated with regard to the size of our split training dataset. }
  \label{table:depth_estimation}
  \centering
  \scalebox{1.0}{
  \begin{tabular}{ll|cc}
    \toprule
    Perc. real (\%) & Perc. gen. (\%) & AbsRel & WHDR \\
    \midrule
    20 & 0 & 0.320 & 0.243 \\
    40 & 0 & 0.257 & 0.205 \\
    60 & 0 & 0.236 & 0.186 \\
    80 & 0 & 0.228 & 0.175 \\
    100 & 0 & 0.218 & 0.165 \\
    0 & 20 & xxx & xxx \\
    20 & 20 & 0.280 & 0.213 \\
    20 & 40 & 0.256 & 0.196 \\
    20 & 60 & 0.245 & 0.185 \\
    20 & 80 & 0.233 & 0.177 \\
    20 & 100 & 0.227 & 0.172 \\
    \bottomrule
  \end{tabular}}
\vspace{-1em}
\end{table}
